Weak Simplicial Bisimilarity for Polyhedral Models and SLCS_eta -- Extended Version

In the context of spatial logics and spatial model checking for polyhedral models -- mathematical basis for visualisations in continuous space -- we propose a weakening of simplicial bisimilarity. We additionally propose a corresponding weak notion of $\pm$-bisimilarity on cell-poset models, a discrete representation of polyhedral models. We show that two points are weakly simplicial bisimilar iff their repesentations are weakly $\pm$-bisimilar. The advantage of this weaker notion is that it leads to a stronger reduction of models than its counterpart that was introduced in our previous work. This is important, since real-world polyhedral models, such as those found in domains exploiting mesh processing, typically consist of large numbers of cells. We also propose SLCS_eta, a weaker version of the Spatial Logic for Closure Spaces (SLCS) on polyhedral models, and we show that the proposed bisimilarities enjoy the Hennessy-Milner property: two points are weakly simplicial bisimilar iff they are logically equivalent for SLCS_eta. Similarly, two cells are weakly $\pm$-bisimilar iff they are logically equivalent in the poset-model interpretation of SLCS_eta. This work is performed in the context of the geometric spatial model checker PolyLogicA and the polyhedral semantics of SLCS.

==> EtaMinimisation.tex <==
\section{Building the Minimal Model Modulo $\slcsEeq$}\label{sec:EtaMinimisation}


In this section we present a finite poset model minimisation procedure, modulo weak \plm-bisimilarity or, equivalently, $\slcsEeq$. The procedure, given  a finite poset model  $\calF = (W, \preceq, \peval)$, proceeds in three steps:\\[1em]
\noindent
{\bf Step 1} $\calF$ is encoded  into a \lts{,}  denoted $\posToltsC(\calF)$.
The set of states of $\posToltsC(\calF)$ is $W$ and it is guaranteed that,
for all $w_1, w_2 \in W$, $w_1$ and $w_2$ are logically equivalent in $\calF$, with respect to \slcsE{,} if and only if they are branching equivalent in $\posToltsC(\calF)$.\\[1em]
\noindent
{\bf Step 2} $\posToltsC(\calF)$ is reduced modulo branching equivalence, using available software tools, like {\tt mCRL2}: 
this step
yields the equivalence classes of $W$ modulo branching equivalence. In other words,
we get $W_{/\slcsEeq^{\calF}}$. \\[1em]
\noindent
{\bf Step 3} The minimal model is built. This model is not necessarily a poset model, but it is
guaranteed to be a reflexive Kripke model $(W_{/\slcsEeq^{\calF}},R)$
where $R$ is a relation induced by $\preceq$.\\[1em]

In the remainder of this section we focus on Step 1 and Step 3. 

\subsection{The $\posToltsC$ encoding}

The definition of the encoding $\posToltsC$ follows:

\begin{definition}\label{def:LTSetaConc}
Given finite poset model $\calF=(W,\preceq,\peval)$, and $\tau,\cact, \dact \notin \ap$,
we define the \lts{} $\posToltsC(\calF) = (S,L,\longrightarrow)$ where
\begin{itemize}
\item
the set $S$ of states is the same as $W$;
\item
the set $L$ of labels is $\ap \cup \SET{\tau,\cact, \dact}$; 
\item
the transition relation is the smallest relation on $W \times L \times W$ induced by the following transition rules:\\
$$
(\mbox{PLC})
\sosrule{w\in \peval(p)}{w\trans{p} w}
\quad\quad\quad
(\mbox{TAU})
\sosrule{w \preceqsucc w', \invpeval(\SET{w})=\invpeval(\SET{w'})}{w\trans{\tau} w'}
$$\\
$$
(\mbox{CNG})
\sosrule{w \preceqsucc w', \invpeval(\SET{w})\not=\invpeval(\SET{w'})}{w\trans{\cact} w'}
\quad\quad\quad
(\mbox{DWN})
\sosrule{w \succeq w'}{w \trans{\dact} w'}
$$
\end{itemize}
\closedefi
\end{definition}

For proving that $w_1 \slcsEeq^{\calF} w_2$ if and only if $w_1 \beq^{\posToltsC(\calF)} w_2$
it is convenient to resort to an intermediate structure, that is in fact another \lts{,} obtained from 
$\calF$ via another encoding. We call  $\posToltsA(\calF)$ this second \lts{}.
%
Suppose now that $w_1$ and $w_2$ are mapped into states  $s_1$ and $s_2$ of $\posToltsA(\calF)$, respectively. 
It turns out  that $w_1$ and $w_2$ are logically equivalent in $\calF$, with
respect to \slcsE{,} if and only if $s_1$ and $s_2$ are strongly equivalent in $\posToltsA(\calF)$.
Furthermore, we have that $s_1$ and $s_2$ are strongly equivalent in $\posToltsA(\calF)$ if and
only if $w_1$ and $w_2$ are branching equivalent in $\posToltsC(\calF)$, which proves the claim.

$\posToltsA(\calF)$ is an abstraction of $\posToltsC(\calF)$. 
Intuitively, let $\Theta =\ZET{\invpeval(\SET{w})}{ w\in W}$ and, 
for $\alpha \in \Theta$, let us consider, 
the $\alpha$-connected components of $\calF$. Then,
each state $s$ of $\posToltsA(\calF)$ is an  $\alpha$-connected component of $\calF$, for some 
$\alpha$ as above. So, we group together all those $w$ that can reach one another only via paths in $\calF$ composed of elements all satisfying the same proposition letters.

The above intuition on the nature of the states of $\posToltsA(\calF)$  is formalised by the following definition:

\begin{definition}\label{def:LCCeq}
Given finite poset model $(W,\preceq,\peval)$, we define relation 
$\lcceq \, \subseteq W \times W$ as the set of pairs $(w_1,w_2)$ such that 
an undirected path $\pi$ of some length $\ell$ exists with
$\pi(0)=w_1, \pi(\ell)=w_2$ and $\invpeval(\SET{\pi(i)})=\invpeval(\SET{\pi(j)})$,
for all $i,j\in [0;\ell]$.
\end{definition}

The following proposition follows directly from the relevant definitions:
%
\begin{proposition}
Let $(W,\preceq,\peval)$ be a  finite poset model.
Relation $\lcceq$ over $W$ is an equivalence relation.\qed
\end{proposition}


We are ready for defining the encoding into the intermediate, more ``abstract'' \lts{:}

\begin{definition}\label{def:LTSetaAbs}
Given finite poset model $\calF=(W,\preceq,\peval)$, and $\sact,\dact \notin \ap$,
we define the \lts{} $\posToltsA(\calF) = (S,L,\longrightarrow)$ where
\begin{itemize}
\item
the set $S$ of states is the quotient $W_{/\lcceq}$ of $W$ modulo $\lcceq$;
\item
the set $L$ of labels is $\pws{\ap} \cup \SET{\sact,\dact}$;
\item
the transition relation is the smallest relation on $W \times L \times W$ induced by the following transition rules:
$$
(\mbox{PL})[w]_{\lcceq} \trans{\invpeval(\SET{w})} [w]_{\lcceq}
$$
$ $\\
$$
(\mbox{Step})\sosrule{w \preceqsucc w'}{[w]_{\lcceq} \trans{\sact} [w']_{\lcceq}}\quad
(\mbox{Down})\sosrule{w \succeq w'}{[w]_{\lcceq} \trans{\dact} [w']_{\lcceq}}
$$
\end{itemize}
\closedefi
\end{definition}

The following theorem ensures  that $w_1$ and $w_2$ are logically equivalent in $\calF$, with
respect to \slcsE{,} if and only if $[w_1]_{\lcceq}$ and $[w_2]_{\lcceq}$ are strongly equivalent in $\posToltsA(\calF)$.

\begin{theorem}\label{thm:StrongEqLogeq}
Let $\calF=(W,\preceq,\peval)$ be a  finite poset model.
For all $w_1,w_2 \in W$ the following holds: 
$[w_1]_{\lcceq} \seq^{\posToltsA(\calF)} [w_2]_{\lcceq}$ iff $w_1 \slcsEeq^{\calF} w_2$.
\end{theorem}


The following theorem ensures that $[w_1]_{\lcceq}$ and $[w_2]_{\lcceq}$ are strongly equivalent in $\posToltsA(\calF)$ if and only if $w_1$ and $w_2$ are branching equivalent in $\posToltsC(\calF)$, thus completing the proof of our claim.

\begin{theorem}\label{thm:StrongEqBranching}
Let $\calF=(W,\preceq,\peval)$ be a  finite poset model.
For all $w_1, w_2 \in W$ the following holds: 
$[w_1]_{\lcceq} \seq^{\posToltsA(\calF)} [w_2]_{\lcceq}$ iff
$w_1 \beq^{\posToltsC(\calF)} w_2$.
\end{theorem}


From Theorem~\ref{thm:StrongEqLogeq}  and  Theorem~\ref{thm:StrongEqBranching} we finally get our claim:

\begin{corollary}\label{cor:LogeqEqBranch}
Let $\calF=(W,\preceq,\peval)$ be a  finite poset model. For all $w_1,w_2 \in W$ the following holds: $w_1 \slcsEeq^{\calF} w_2$ iff $w_1 \beq^{\posToltsC(\calF)} w_2$.
\end{corollary}

We have now characterised the equivalence classes of logical equivalence  $\slcsEeq$
on the carrier of a poset model $\calF$ as the same as those of branching equivalence
$\beq$ on the set of states of $\posToltsC(\calF)$ and we can compute the latter
by means of a tool for branching equivalence minimisation, e.g., {\tt mCRL2}.


\subsection{Building the minimal model}

In this section we show how to build the minimal model, modulo $\slcsEeq$, once we have
computed the equivalence classes.
Below we define the minimal model:
%
\begin{definition}[$\calF_{\min}$]\label{def:MinE} 
For finite poset model $\calF=(W,\preceq,\peval)$ let 
$\calF_{\min}$ be defined as 
$\calF_{\min} = (W_{\min},R_{\min},\peval_{\min})$ where
\begin{itemize}
\item $W_{\min} = W_{/\slcsEeq}$;
\item $R_{\min}=
\ZET{(\alpha_1,\alpha_2) \in W_{\min} \times W_{\min}}{\mbox{there are } w_1\in \alpha_1, w_2 \in \alpha_2 \mbox{ s.t. } w_1 \preceq w_2}$;
\item $\peval_{\min}(p) = \ZET{\alpha \in W_{\min}}{\mbox{there is } w \in \alpha \mbox{ s.t. } w\in   \peval (p)}$, for each $p \in \ap$.
%$ $\\\vspace{-0.3in}
%\closedefi	\\
\end{itemize}
\closedefi
\end{definition}
%
Clearly, $R_{min}$ is a reflexive relation since $\preceq$ is a partial order. Furthermore it is minimal with respect to \slcsE{} by definition of $\slcsEeq$ and $W_{/\slcsEeq}$. The following theorem ensures that the model defined above is sound and complete with respect to the logic, so that the minimisation procedure is correct.

%
\begin{theorem}\label{theo:MinE}
Given finite poset model $\calF=(W,\preceq,\peval)$ let 
$\calF_{\min}$ be defined as in Definition~\ref{def:MinE}.
Then, for each $w \in W$ and \slcsE{} formula $\form$ the following holds:
$
\calF,w \models \form \mbox{ iff } 
\calF_{\min}, [w]_{\slcsEeq} \models \form.
$
\end{theorem}


\diego{We should consider moving Example~\ref{exa:MinRunExaE} here.}












